Cross-Sections for $\text{t}\bar{\text{t}}\text{H}$ production with the Top Quark $\overline{\text{MS}}$ Mass

We study the impact of the top quark mass renormalized in the $\overline{\text{MS}}$ scheme on the $\text{t}\bar{\text{t}}\text{H}$ production cross-sections as an alternative to theory predictions with the conventionally used pole mass scheme. The differential cross-sections at next-to-leading order in perturbative QCD with stable top quarks show a moderate decrease in scale uncertainties for the $\overline{\text{MS}}$ mass renormalization scheme compared to the on-shell one. The shape of the differential distributions is not affected much, the largest differences being observed in the invariant mass distributions of the $\text{t}\bar{\text{t}}$ and the $\text{t}\bar{\text{t}}\text{H}$ systems.

==> Content/MassDerivative.tex <==
%% ===========================
\section{Estimation of Mass Derivative of the Born-Level Cross-Section}
\label{ch:PhenomenologyttH:sec:MassDerivative}
%% ===========================

Since the Born-Level cross-section of the \ttbarH\ production process is known in the pole mass scheme, it is used to estimate the effect of the top quark running mass on the differential cross-sections numerically.
It is compelling to study the behavior of the top quark and the Higgs boson separately, as well as the behavior of systems of particles.
Therefore, the distributions investigated in this study are the transverse momentum \pT\ and the rapidity $y$ of the top quarks and the Higgs boson, as well as  the invariant mass of the top quark pair and the \ttbarH\ system.

To estimate the derivative of the Born-Level cross-section, \\\MGaMCatNLOOnly\ \cite{Alwall:2014hca}(version 2.6.5) is used to simulate the differential cross-sections varying the the mass of the top quark (and the Yukawa coupling accordingly) between $\mTop=150$ \GeV\ and $\mTop=175$ \GeV\ in steps of $\Delta \mTop=0.5$ \GeV.
The calculations are performed using the $\textsc{MMHT2014}$ PDF sets \cite{Harland-Lang:2014zoa} with $\alphas(m_\aZ)=0.118$.
The \msbar\ mass of the top quark at the scale $\mTop$ is chosen to be $\mTop(\mTop) = 163.2$ \GeV, while the corresponding pole mass is $\PoleMass=172.5$ \GeV.
The mass of the Higgs boson is chosen to be $\HiggsMass = 125.0$ \GeV.
To calculate the differential cross-sections of the \ttbarH\ production in the \msbar\ scheme from Equation \ref{eq:DiffXSmsbar}, the running of \alphas\ and the top quark mass are calculated in the \emph{5FNS} using the RunDec software \cite{Chetyrkin:2000yt,Schmidt:2012az}.

Calculating differential cross-sections in steps of $\Delta \mTop=0.5$ creates a two-dimensional distribution as a function of the observable $X$ and the mass of the top quark.
Figure \ref{fig:BornDerivative2d} illustrates this distribution for the \pT\ and the $y$ of the top quarks.

\begin{figure}[htp]
	\centering
	\includegraphics[width=.9\textwidth]{Figures/MassDerivative/MassDependenceRoot.png}
	
	\caption{\label{fig:BornDerivative2d} Two dimensional histogram for the estimation of the derivative of the Born-level cross-section. 
		The transverse momentum of the Higgs boson in the \ttbarH\ process is simulated as a function of top quark mass between $\mTop=150$ \GeV\ and $\mTop=175$ \GeV\ in the pole mass renormalization scheme. }
\end{figure}

Since the derivative is estimated numerically, low statistical precision on the Born-level differential cross-sections will lead to large statistical uncertainties on the final result.
Therefore, each of the cross-sections as a function of \mTop\ is calculated with a statistical precision of $0.1\text{\textperthousand}$ on the total cross-section to ensure low statistical uncertainty of the Born derivative in each bin. 
The cross-sections in the pole mass scheme at the NLO precision are calculated with $0.2\text{\textperthousand}$ statistical uncertainty requirement on the total cross-section.
Afterwards, the mass derivative of the Born-level cross-section is estimated with the difference in cross-section in each bin of the differential distribution when going from $\mTop\rightarrow \mTop+\Delta \mTop$, as is shown in Equation \ref{eq:derivative}. 

\begin{align}
	\label{eq:derivative}
	\frac{d}{d \mTop}\left(\frac{d \sigma^{(0)}\left(\mTop\right)}{d X}\right) \approx \frac{\frac{d \sigma^{(0)}\left(\mTop + \Delta m\right)}{d X} - \frac{d \sigma^{(0)}\left(\mTop\right)}{d X}}{\Delta m}
\end{align} 

Having estimated the Born-level derivative, Equation \ref{eq:DiffXSmsbar} is used to obtain the differential cross-sections of \ttbarH\ production in the \msbar\ scheme.
For the calculation of the scale uncertainties of the predictions, \muR\ and \muF\ are varied between $[0.5\cdot\mu_0,2\cdot\mu_0]$.% and, thus, the \MSbarMass\ accordingly.
The top quark \msbar\ mass $\mTop(\mTop)$ is kept unchanged between the scale variations.
Due to the requirement on the numerical precision of the cross-sections, the statistical uncertainties on the mass derivative are negligible in the bulk of the distributions.
However, for the transverse momentum and invariant mass distributions, the statistical uncertainties become relevant in the region of $\gtrapprox 1$ \TeV.
Consequently, the binning of the distributions is chosen to keep the statistical uncertainties small compared to the scale uncertainties.
Despite being small, the statistical uncertainties on the Born-level derivative are added in quadrature to the scale uncertainties to stay consistent.
